ARTIST: ARTificial Intelligence for Simplified Text

Complex text is a major barrier for many citizens when accessing public information and knowledge. While often done manually, Text Simplification is a key Natural Language Processing task that aims for reducing the linguistic complexity of a text while preserving the original meaning. Recent advances in Generative Artificial Intelligence (AI) have enabled automatic text simplification both on the lexical and syntactical levels. However, as applications often focus on English, little is understood about the effectiveness of Generative AI techniques on low-resource languages such as Dutch. For this reason, we carry out empirical studies to understand the benefits and limitations of applying generative technologies for text simplification and provide the following outcomes: 1) the design and implementation for a configurable text simplification pipeline that orchestrates state-of-the-art generative text simplification models, domain and reader adaptation, and visualisation modules; 2) insights and lessons learned, showing the strengths of automatic text simplification while exposing the challenges in handling cultural and commonsense knowledge. These outcomes represent a first step in the exploration of Dutch text simplification and shed light on future endeavours both for research and practice.

==> sections/limitations.tex <==
\section{Limitations of Language Models} \label{sec:limitations}
\lore{Limitations; injection of new facts}

Most natural language translators in the field use language models in various sizes. The GPT-3 translator~\cite{NEURIPS2020_1457c0d6} for example shows its capabilities by inserting certain facts related to some knowledge domain such as astronomy, to simplify and summarise larger and more complex texts. Consider the following complex text:
\begin{quote}
\em{Jupiter is the fifth planet from the Sun and the largest in the Solar System. It is a gas giant with a mass one-thousandth that of the Sun, but two-and-a-half times that of all the other planets in the Solar System combined. Jupiter is one of the brightest objects visible to the naked eye in the night sky, and has been known to ancient civilisations since before recorded history. It is named after the Roman god Jupiter. When viewed from Earth, Jupiter can be bright enough for its reflected light to cast visible shadows, and is on average the third-brightest natural object in the night sky after Mercury, the Moon and Venus.}
\end{quote}
Compare this with its simplification, and appreciate the highlight indication additional information not found in the original text:
\begin{quote}
\em{Jupiter is the fifth planet from the Sun and the largest in the Solar System. It is a gas giant {\bf made of hydrogen and helium}. Jupiter is one-thousandth the size of the Sun, but two and a half times the size of all the other planets in the Solar System combined. It is very bright and can be seen in the night sky.}
\end{quote}

A number of ex-Google employees \citep{exgoogle} discussed the ethical, sometimes toxic consequences of using text produced by language models (LMs).
They stressed that existing language models behave like ``parrots'', repeating what they learned without knowing the meaning nor the possible consequences of what they generate.
Ignoring the limitations of such models incurs the danger of toxic outputs being generated and unwanted consequences.
% They stressed that the size of the language model (LM) used by some parrot system (read: automated natural language translator repeating what it learned, not knowing the meaning nor possible consequences) increases the danger of toxic translations resulting in getting innocent people accused for humiliation or terrorising intentions.

\lore{Another part which I do not understand...}
Several papers report methods -- among one the CESI method \cite{vashishth2018cesi} -- how to build up language models from documents automatically or semi-automatically. These papers stress the human factor for building up these models as labour-intensive. By reducing the human factor, the creation of their large LMs and use can induce unwanted errors.

We invented the concept of building up language models from documents automatically using some heuristics as a first step, followed by a second semi-automatic supported by a manual correction step to convert these complex LMs to more simplified versions. These simplified LMs corresponds to standardised language comprehension reading levels. In our proposed pipeline these LMs are used for correction of simplified texts translated by existing translators. How this LM is created is one of our research questions.

Nonetheless, language models can behave like collections of information found in ontologies, knowledge graphs, vocabularies or lexicons. Figure \ref{fig:ontology} shows a possible ontology in line with the example given above.

\begin{figure}[t]
\includegraphics[width=0.45\textwidth]{images/SolarSystem.PNG}
\caption{Ontology example of the solar system. From this description of knowledge, word combinations can be derived and inserted in texts.}
\label{fig:ontology}
\end{figure}

==> sections/related.tex <==
\section{Background and Related Work} \label{sec:related}

\iffalse
Within the ICT with Industry workshop, several researchers work on use cases provided by the industry. The use case 'ARTificial Intelligence for Simplified Text' was provided by KB, the National Library of the Netherlands.

\subsection{About KB}
The KB, the National Library of the Netherlands, collects and stores all written publications that appear in the Netherlands and makes them available to all Dutch citizens. This includes books, newspapers and periodicals, but also websites and e-books. The KB is one of the largest cultural heritage institutions in the Netherlands and its research department focuses on topics ranging from providing insights into the development of the public library sector to applying AI techniques to open up our collections to a wide audience. The KB is an active player in the field of Artificial Intelligence: it is co-founder of the Cultural AI Lab and the working group Culture \& Media of the Netherlands AI Coalition.
\fi

% \subsection{Studies on Literacy} \label{sec:audiences}

Literacy is defined as ``the ability to understand and respond appropriately to written texts'', and forms a key information processing competency \citep{oecd2019survey}.
% Whatever the cause (language barriers, cognitive difficulties, or being in a state of cognitive development), having a basic literacy level is defined as being able to read texts of a short length and find explicit information to make partial inferences \citep{aluisio2010readability}. 
Embedded clauses, passive voice, non-canonical word order, and low-frequency words can disrupt the sequential order of sentences \citep{gasperin2009natural}.
% To that aim, a good text simplification (TS) strategy should avoid producing an output with long, complex and conjoined sentences.
% Embedded clauses, use of the passive voice, non-canonical word order and low-frequency words should also be stripped, making the sequential order of sentences easier to follow \citep{gasperin2009natural}.
In this sense, resources like corpus-specific frequency lists \citep{bauman1995general}, controlled languages such as ASD-STE100\footnote{ASD-STE100: \url{https://asd-ste100.org/about.html}}, and guidelines for accessible communication \citep{ukgov2022accessible} have been developed.
% For example, corpus-based frequency lists \citep{bauman1995general} could be used to count low-frequency words; or a controlled language such as ASD-STE100\footnote{ASD-STE100: \url{https://asd-ste100.org/about.html}} (simplification of English maintenance instructions) could be used to discard those words.
%
% When dealing with long publications, a simple strategy would be to split the text into more digestible chunks.
% Further, the UK Government’s Accessible Communication Formats guidance \citep{ukgov2022accessible} advises splitting any text which is longer than 24 pages into composite parts, have sentences only contain 10-15 words and describe one main idea or context and one verb, and --- for technical materials --- have acronyms expanded at least once.
%
To that aim, generative AI models can be the starting point of TS strategies, providing human experts with an initial draft.

% \par{\textbf{Different Causes Call for Different TS Strategies}}
Unsurprisingly, different causes call for different TS strategies.
For example, the OECD reported that immigrant communities in the Netherlands generally have lower levels of Dutch language proficiency \citep{oecd2019survey}.
% This is a reflection of the high level of literacy among the Dutch-born population and not necessarily the low literacy of immigrant communities.
For those with a mastery of a language other than Dutch, reading is complicated by vocabulary loads, linguistic structure and discourse style \citep{candido2009supporting}.
% These factors act as a barrier to the reader’s already-present knowledge of the language interacting with the content and context of the text.
% ‘When these factors do not match the reader’s knowledge and experience, the text becomes too complex for comprehension to occur’ \citep{candido2009supporting}.
% In this case, a model which translates Dutch into a target language like English could be beneficial.
%
% Furthermore, for adult readers with cognitive impairments, such as dyslexia, a full-fledged TS solution should also account for alternative output layouts (typefaces, glossaries, pictures, etc.).
Furthermore, cognitive impairments (e.g., dyslexia) require alternative output layouts (typefaces, glossaries, pictures, etc.).
%
Instead, for materials directed at readers in a state of cognitive development, it is desirable to have a vocabulary which can be phonetically sounded and decoded to forming sound-symbol correspondences. % and ideas of meaning.
% For child readers, shorter and simpler words should be opted for.
Prepositions, words denoting sequences, classifications (e.g., concerning animals), are all essential to cognitive and reading development and should be retained.
% 
% A sans-serif font, like Arial, should be used, with larger font and greater spacing. Text should also commonly be aligned to the left. An automatically generated glossary of terms would also be beneficial, to lessen any jargon missed by the TS model. `Flow charts are ideal for explaining procedures. Pictograms and graphics can help locate and support information’. %\todo{(link to Richard’s flowchart)}.
% Conversely, simpler pictorial references, complete with alternative text, may be more suitable for a younger audience.
Needless to say, consultation with these groups is necessary to validate any TS solution.
% There should be ample opportunities for the KB to conduct data-gathering activities, with the library hosting 25,000 children activities and 32,000 language learning activities in 2018 alone.\footnote{Koninklijke Bibliotheek, ‘Libraries are attracting more visitors’, accessed 18 January, 2022. \url{https://www.kb.nl/en/news/2019/libraries-are-attracting-more-visitors}}

\par\textbf{Text simplification} (TS) is a long-standing task in NLP, attracting  continuous interest from the research community \citep{sheang2021controllable,al2021automated}.
In the last few decades, methods for both lexical and syntactic simplification have been developed; from rule-based to data-driven approaches \citep{glavavs2015simplifying,horn2014learning,specia2010translating}.
% In contrast to rule-based methods, that require manual input from trained human editors, data-driven methods extract text simplification rules automatically from training corpora.
In particular, data-driven methods has focused on neural methods capable of capturing the distributional semantics of words \citep{mikolov2013distributed, devlin2018bert}, a key requirement for meaning preservation and text coherence.
Correspondingly, a visible trend in TS is the recent shift from statistical machine translation, from, e.g., phrase-based approaches \citep{koehn2007moses} to neural machine translation \citep{wang2016experimental, zhang2017sentence}.
Neural TS methods are at the early stage and are still found to be unreliable, often capturing spurious or biased correlations.
% and are hard to explain, due to linear and non-linear data transformation incomprehensible to humans.
The problem is more obvious when large training data does not exist, a common situation in resource-limited languages such as Dutch.
% In high-stakes domains with safety, trust, or ethical requirements, the aforementioned limitations of neural models can lead to negative and sometimes damaging effects.
% In this report, we explore TS in Dutch to gain an understanding of the challenges and shed light on future research directions.
%
% \subsection{Lexical Text Simplification}
% Not much work has been done on algorithmic text simplification for the Dutch language, according to our knowledge.
Limited efforts have been done for Dutch TS.
For instance, \citet{bulte2018automating} identify difficult words by cross-checking their age of acquisition --- as frequent words are usually learnt at a young age \citep{moors2013norms}---, frequency in the Wablieft corpus \citep{vandeghinste2019wablieft}, and definitions from Dutch Wikiepdia.
% In particular, age of acquisition was found to be negatively correlated with word frequency \citep{moors2013norms}, i.e., frequent words are learnt early on.
% Based on this, simple synonyms are then extracted from the Cornetto database \citep{piek2013cornetto}.
Another aspect to consider is the abstractness of concepts.
In this sense, T-scan \citep{pander2014t} builds on top of a Dutch lexical database \citep{maks2005eferentie,rbn2014referentie} which compiles 50.000 semantic types for nouns, verbs, adjectives, and adverbs.

% with a long-term ambition to address aforementioned challenges by investigating new approaches from a wide range of angles such as data, modelling, and humans in the loop for TS evaluation, interpretation, and improvement.





 


==> sections/z-OLD-data.tex <==
\section{Data} \label{sec:data}

\lore{Removed. Didn't use this.}
For this workshop we use training data on three levels of complexity from the `Canon van Nederland'.
These texts were used by \cite{pander2017onderwijsteksten} in their research for simplifying educational texts. The Dutch canon offers 50 short texts that teach Dutch school children in primary and secondary education about important parts of Dutch culture and history. Because the texts are provided at three different levels of complexity, they are useful in our research on text simplification, and in particular for fine tuning the bidirectional transformer model we use.
The editors of the `Canon van Nederland' have given us permission to use this data.

The texts are each connected to a single item from the Canon. The three levels of complexity correspond to reading skills that are linked to children in groups 5 and 6 of primary education, and with those of children in the lower and upper classes of secondary school. With these parallel texts we can train/fine tune an automatic text simplification model with which we are ultimately able to 'translate' complex texts into simpler texts.

Since the individual texts on the three different levels cannot be regarded as parallel texts in all respects, they have been compared and edited to align them. This is done manually.
The alignment of the texts can be done sentence-wise or paragraph-wise. Paragraph alignment was chosen in this study, partly because substantive similarities between the parallel texts are easier to distinguish in these texts. Sentences that correspond substantively appear in various places within the paragraphs, which makes sentence alignment too complex. In addition, care must be taken to preserve grammatical fluency and preservation of meaning in a text paragraph.

% \todo{}
% \note{Here we describe the datasets we experimented with and that we build. We need to report on whether we can share our Canon van Nederland data.}

==> sections/z-OLD-lexical.tex <==
\section{Lexical Simplification}
\label{sec:lexical}
\lore{Related works; Dutch as a low-resource language}

Not much work has been done on algorithmic text simplification for the Dutch language. According to our knowledge. 
% the only work lexical text simplification for Dutch was done by \citet{bulte2018automating}.
\citet{bulte2018automating} identify difficult words by cross-checking their age of acquisition \lore{ref?}, their frequency in the Wablieft corpus \lore{ref!}, and definitions from Dutch Wikiepdia.
In particular, age of acquisition was found to be negatively correlated with word frequency \citep{moors2013norms}, i.e., frequent words are learnt early on.
Based on this, simple synonyms are extracted from the Cornetto \lore{ref!} database.
Another aspect to consider is the concreteness (or abstractness) of concepts.
In this sense, T-scan \citep{pander2014t} builds on top of a Dutch lexical database \citep{maks2005eferentie,rbn2014referentie} which compiles 50.000 semantic types for nouns, verbs, adjectives, and adverbs.

% Their approach consists of multiple steps. They identify difficult words based on the average age one would acquire the word and the frequency of the word based on the Wablieft corpus, including weekly newspapers. Another important step is the identification of appropriate, simpler synonyms. 
% Bulté et al. uses the proprietary Cornetto database, consisting of synsets and their relationships to each other.
% Their simplification pipeline also includes preprocessing, validation and of the data augmentation.
% The augmentation is based on the Dutch Wikipedia to append definitions to complicated words.

%#### TODO: First give an overview (frequency for difficulty, then BERTje for replacements) and explain both in more detail).

\lore{Don't know what this is supposed to mean}
We experimented with the Dutch variant of BERT \citep{devlin2018bert}, named BERTje \citep{de2019bertje}, to identify complex words and use word frequency information from various sources to replace these complex words by more frequent synonyms that are possibly easier to understand.

% On the relation between word frequency and ease of understanding
% The intuition that the usage frequency of words is related to the age at which children learn words is born out by empirical research. \citet[p. 174]{moors2013norms} investigated the age of acquisition of a set of 4300 (mostly emotion-related) words and found a strong negative correlation between word frequency and age of acquisition. In other words, frequent words are learned earlier on. 

Apart from word frequency, the concreteness or abstractness of concepts may play a role in how easy they are to understood when used in a text. 
The Dutch lexical reference database contains information on semantic types for 50,000 Dutch nouns, verbs, adjectives and adverbs \citep{maks2005eferentie,rbn2014referentie}. For adjectives, one of the semantic categories is {\em abstract}. This is implemented in T-scan \citep{pander2014t}, so can be operationalised without too much effort.


==> sections/z-OLD-recommendations.tex <==
\section{Recommendations from Focus Group}
\label{sec:audiences}

Literacy is defined as `the ability to understand and respond appropriately to written texts', and forms a key information processing competency \citep{oecd2019survey}.
% Whatever the cause (language barriers, cognitive difficulties, or being in a state of cognitive development), having a basic literacy level is defined as being able to read texts of a short length and find explicit information to make partial inferences \citep{aluisio2010readability}. 
To that aim, a good text simplification (TS) strategy should avoid producing an output with long, complex and conjoined sentences.
Embedded clauses, use of the passive voice, non-canonical word order and low-frequency words should also be stripped, making the sequential order of sentences easier to follow  \citep{gasperin2009natural}.
For example, corpus-based frequency lists \citep{bauman1995general} could be used to count low-frequency words; or a controlled language such as ASD-STE100\footnote{ASD-STE100: \url{https://asd-ste100.org/about.html}} (simplification of English maintenance instructions) could be used to discard those words.

\par{\textbf{Different Causes Call for Different TS Strategies}}
Perhaps unsurprisingly, the OECD reported that immigrant communities in the Netherlands generally have lower levels of Dutch language proficiency \citep{oecd2019survey}.
This is a reflection of the high level of literacy among the Dutch-born population and not necessarily the low literacy of immigrant communities.
For those with a mastery of a language other than Dutch, reading is complicated by vocabulary loads, linguistic structure and discourse style \citep{candido2009supporting}.
% These factors act as a barrier to the reader’s already-present knowledge of the language interacting with the content and context of the text.
% ‘When these factors do not match the reader’s knowledge and experience, the text becomes too complex for comprehension to occur’ \citep{candido2009supporting}.
% In this case, a model which translates Dutch into a target language like English could be beneficial.
%
Furthermore, for adult readers with cognitive impairments, such as dyslexia, a full-fledged TS solution should also account for alternative output layouts (typefaces, glossaries, pictures, etc.).
% A sans-serif font, like Arial, should be used, with larger font and greater spacing. Text should also commonly be aligned to the left. An automatically generated glossary of terms would also be beneficial, to lessen any jargon missed by the TS model. `Flow charts are ideal for explaining procedures. Pictograms and graphics can help locate and support information’. %\todo{(link to Richard’s flowchart)}.
% Conversely, simpler pictorial references, complete with alternative text, may be more suitable for a younger audience.
Needless to say, consultation with these three groups will be necessary to ensure that any TS meets the needs of semi-literate readers.
% There should be ample opportunities for the KB to conduct data-gathering activities, with the library hosting 25,000 children activities and 32,000 language learning activities in 2018 alone.\footnote{Koninklijke Bibliotheek, ‘Libraries are attracting more visitors’, accessed 18 January, 2022. \url{https://www.kb.nl/en/news/2019/libraries-are-attracting-more-visitors}}

\par{\textbf{Readers, Context, and Use Cases}}
Text Simplification systems are a prime example of how readers' needs, context, and application context matter.
A simple strategy for long publications, such as fiction books, would be to split texts into smaller parts.
% For long publications, such as dense fiction and non-fiction, opposed to shorter materials such as websites or reports, it would be beneficial to factor the splitting of texts into smaller parts into any TS strategy.
For instance, the UK Government’s Accessible Communication Formats guidance \citep{ukgov2022accessible} advises splitting any text which is longer than 24 pages into composite parts, have sentences that only contain 10-15 words and describe one main idea or context and one verb.
Further, for technical materials, acronyms should be expanded (at least at the first point of use). This corroborates that text simplification is different from summarisation and does not necessarily entail overall shorter texts.
% In terms of visualisations, the use of shapes and contrasting colours is also advised.
A concrete example is given in a survey by the OECD \citep{oecd2019survey}: 18\% of 15-year-olds cannot understand the content of municipality letters\footnote{CEDEFOP, ‘Netherlands: Poor literacy among teens on the rise’: \url{https://www.cedefop.europa.eu/en/news/netherlands-poor-literacy-among-teens-rise}}.
%
% Looking at young adults (16-24), seen by the OECD as having a higher average of literacy than the rest of the Dutch population \citep{oecd2019survey}, government records still need to be simplified: with a Court of Audit report (2016), commissioned by the Foundation for Reading and Writing, finding that 18\% of 15-year-olds cannot understand the content of municipality letters.\footnote{CEDEFOP, ‘Netherlands: Poor literacy among teens on the rise’, accessed 18 January, 2022. \url{https://www.cedefop.europa.eu/en/news/netherlands-poor-literacy-among-teens-rise}}
%
In the case of materials directed at younger readers in a state of cognitive development, the use of vocabulary which can be phonetically sounded and decoded (forming sound-symbol correspondences and ideas of meaning) should be retained.
For child readers, shorter and simpler words should be opted for.
Prepositions (under/over etc.), words denoting sequences such as size, classifications (for instance concerning animals), are all essential to cognitive and reading development and should remain in the text.

==> sections/z-OLD-visualisation.tex <==
\section{Visualisation}
\label{sec:visualisation}
\lore{Remove, swap for implementation}

Simplification of texts to certain reading levels are usually expressed into a textual format. This format can also be supported by visualisations such as mind maps, graph presentations or the use of pictographs or even pictures of everyday situations, to improve its understanding.

As an example we show in figure \ref{fig:mindmap} a complex text and the corresponding simplified version embedded into a mind map visualisation. Here the noun- and verb phrases are the components to build up the mind map. A research study about developing a dietary supplement knowledge graph done by \cite{xinghe2019aloha} shows that visualisations of texts decrease the reading comprehension level compared to texts automatically simplified by current available translators and presented traditionally. We must report however that the simplified textual formatted version created manually has a slightly lower reading comprehension level compared to both.

\begin{figure}[ht]
\includegraphics[width=0.45\textwidth]{images/Text2MindMap.PNG}
\caption{Traditional and novel mind map presentation of a simplified text. Made with the website \url{https://tobloef.com/text2mindmap/}}
\label{fig:mindmap}
\end{figure}


